A Simple Approach to Jointly Rank Passages and Select Relevant Sentences in the OBQA Context

In the open book question answering (OBQA) task, selecting the relevant passages and sentences from distracting information is crucial to reason the answer to a question. HotpotQA dataset is designed to teach and evaluate systems to do both passage ranking and sentence selection. Many existing frameworks use separate models to select relevant passages and sentences respectively. Such systems not only have high complexity in terms of the parameters of models but also fail to take the advantage of training these two tasks together since one task can be beneficial for the other one. In this work, we present a simple yet effective framework to address these limitations by jointly ranking passages and selecting sentences. Furthermore, we propose consistency and similarity constraints to promote the correlation and interaction between passage ranking and sentence selection.The experiments demonstrate that our framework can achieve competitive results with previous systems and outperform the baseline by 28\% in terms of exact matching of relevant sentences on the HotpotQA dataset.

==> tables/HotpotQA_examples.tex <==
\begin{table}[t]
\small
    \centering
    \small
    \renewcommand{\arraystretch}{1.2}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{|p{0.9\columnwidth}|}
            \hline
                \textbf{Question}: The football manager who recruited David Beckham managed Manchester United during what timeframe?\\
                \textbf{Passage1, 1995–96 Manchester United F.C. season}: The1995-96 season was Manchester United's fourth season in the Premier League, and their 21st consecutive season in the top division of English football. United finished the season by becoming the first English team to win the Double (league title and FA Cup) twice. \textit{Their triumph was made all the more remarkable by the fact that Alex Ferguson had sold experienced players Paul Ince, Mark Hughes and Andrei Kanchelskis before the start of the season, and not made any major signings.Instead, he had drafted in young players like Nicky Butt, David Beckham, Paul Scholes and the Neville brothers, Gary and Phil.}\\
                \textbf{passage2, Alex Ferguson}: \textit{Sir Alexander Chapman Ferguson,CBE (born 31 December 1941) is a Scottish former football manager and player who managed Manchester United from1986 to 2013.} He is regarded by many players, managers and analysts to be one of the greatest and most successful managers of all time.\\
                \textbf{Answer}: from 1986 to 2013\\
                \textbf{Supporting facts}: [["1995-96 Manchester United F.C.season",2],["1995-96 Manchester United F.C. season",3],["AlexFerguson",0]]\\
            \hline
            \end{tabular}
        }
    \caption{Word-level operations to inject noise in each input sequence. Each operation is randomly applied to input sequences with a certain probability $p$.}
    \label{ref: word_operations}
\end{table}
